Safe LLM-Controlled Robots with Formal Guarantees via Reachability Analysis

The deployment of Large Language Models (LLMs) in robotic systems presents unique safety challenges, particularly in unpredictable environments. Although LLMs, leveraging zero-shot learning, enhance human-robot interaction and decision-making capabilities, their inherent probabilistic nature and lack of formal guarantees raise significant concerns for safety-critical applications. Traditional model-based verification approaches often rely on precise system models, which are difficult to obtain for real-world robotic systems and may not be fully trusted due to modeling inaccuracies, unmodeled dynamics, or environmental uncertainties. To address these challenges, this paper introduces a safety assurance framework for LLM-controlled robots based on data-driven reachability analysis, a formal verification technique that ensures all possible system trajectories remain within safe operational limits. Our framework specifically investigates the problem of instructing an LLM to navigate the robot to a specified goal and assesses its ability to generate low-level control actions that successfully guide the robot safely toward that goal. By leveraging historical data to construct reachable sets of states for the robot-LLM system, our approach provides rigorous safety guarantees against unsafe behaviors without relying on explicit analytical models. We validate the framework through experimental case studies in autonomous navigation and task planning, demonstrating its effectiveness in mitigating risks associated with LLM-generated commands. This work advances the integration of formal methods into LLM-based robotics, offering a principled and practical approach to ensuring safety in next-generation autonomous systems.

==> Sections/fig/fig2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,363); %set diagram left start at 0, and has height of 363

%Shape: Polygon [id:ds04415064692387216] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (141,96) -- (162,116) -- (152,140) -- (127,181) -- (108,157) -- (86,116) -- cycle ;
%Shape: Polygon [id:ds5903952103723746] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (206,131) -- (256,161) -- (235.44,193.9) -- (206,241) -- (176,221) -- (156,161) -- cycle ;
%Straight Lines [id:da7490778074815305] 
\draw    (133,132) -- (183.3,162.95) ;
\draw [shift={(185,164)}, rotate = 211.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(133,132)}, rotate = 31.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Shape: Regular Polygon [id:dp7733920429932248] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.41 ] (305,156.5) -- (276.32,195.97) -- (229.93,180.89) -- (229.93,132.11) -- (276.32,117.03) -- cycle ;
%Straight Lines [id:da5203918748551073] 
\draw    (242,166) -- (214.98,214.25) ;
\draw [shift={(214,216)}, rotate = 299.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(242,166)}, rotate = 119.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;

% Text Node
\draw (103,123.4) node [anchor=north west][inner sep=0.75pt]    {$\hat{R}_{0}$};
% Text Node
\draw (200,172.4) node [anchor=north west][inner sep=0.75pt]    {$\hat{R}_{1}$};
% Text Node
\draw (256,135.4) node [anchor=north west][inner sep=0.75pt]    {$X_{obs}$};
% Text Node
\draw (240,202) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{68.49pt}\setlength\topsep{0pt}
\begin{center}
collision check
\end{center}

\end{minipage}};
% Text Node
\draw (159,131.4) node [anchor=north west][inner sep=0.75pt]    {$u_{0}$};


\end{tikzpicture}


==> Sections/fig/fig3.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,363); %set diagram left start at 0, and has height of 363

%Shape: Polygon [id:ds9298070553035973] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (141,96) -- (162,116) -- (152,140) -- (127,181) -- (108,157) -- (86,116) -- cycle ;
%Shape: Polygon [id:ds9420719885971394] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 80; green, 227; blue, 194 }  ,fill opacity=1 ] (187.93,157.89) -- (237.93,187.89) -- (217.36,220.79) -- (187.93,267.89) -- (157.93,247.89) -- (137.93,187.89) -- cycle ;
%Straight Lines [id:da24092747387674573] 
\draw    (133,132) -- (171.99,183.21) ;
\draw [shift={(173.2,184.8)}, rotate = 232.72] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
\draw [shift={(133,132)}, rotate = 52.72] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Shape: Regular Polygon [id:dp7687350550213035] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.41 ] (305,156.5) -- (276.32,195.97) -- (229.93,180.89) -- (229.93,132.11) -- (276.32,117.03) -- cycle ;

% Text Node
\draw (103,123.4) node [anchor=north west][inner sep=0.75pt]    {$\hat{R}_{0}$};
% Text Node
\draw (181,208.4) node [anchor=north west][inner sep=0.75pt]    {$\hat{R}_{1}$};
% Text Node
\draw (256,135.4) node [anchor=north west][inner sep=0.75pt]    {$X_{obs}$};
% Text Node
\draw (154,143.4) node [anchor=north west][inner sep=0.75pt]    {$u_{0}$};


\end{tikzpicture}

